VideoExpert: Augmented LLM for Temporal-Sensitive Video Understanding

The core challenge in video understanding lies in perceiving dynamic content changes over time. However, multimodal large language models struggle with temporal-sensitive video tasks, which requires generating timestamps to mark the occurrence of specific events. Existing strategies require MLLMs to generate absolute or relative timestamps directly. We have observed that those MLLMs tend to rely more on language patterns than visual cues when generating timestamps, affecting their performance. To address this problem, we propose VideoExpert, a general-purpose MLLM suitable for several temporal-sensitive video tasks. Inspired by the expert concept, VideoExpert integrates two parallel modules: the Temporal Expert and the Spatial Expert. The Temporal Expert is responsible for modeling time sequences and performing temporal grounding. It processes high-frame-rate yet compressed tokens to capture dynamic variations in videos and includes a lightweight prediction head for precise event localization. The Spatial Expert focuses on content detail analysis and instruction following. It handles specially designed spatial tokens and language input, aiming to generate content-related responses. These two experts collaborate seamlessly via a special token, ensuring coordinated temporal grounding and content generation. Notably, the Temporal and Spatial Experts maintain independent parameter sets. By offloading temporal grounding from content generation, VideoExpert prevents text pattern biases in timestamp predictions. Moreover, we introduce a Spatial Compress module to obtain spatial tokens. This module filters and compresses patch tokens while preserving key information, delivering compact yet detail-rich input for the Spatial Expert. Extensive experiments demonstrate the effectiveness and versatility of the VideoExpert.

==> Figures/Random_Seed.tex <==
%%
%%

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{Photo/Random_Seed_5.pdf}
  \caption{{Statistical results over 5 independent training instances with different random seeds. Each instance is evaluated 10 times at the same checkpoint.}}
  \label{fg_randomseed}
  \vspace{-0.3 cm}
\end{figure}

==> Figures/Visualization.tex <==
%%
%%

\begin{figure*}[!t]
  \centering
  \includegraphics[width=1\textwidth]{Photo/Visualization_6.pdf}
  \caption{Visualization of joint moment retrieval and highlight detection on QVHighlights dataset.}
  \label{fg_visualization}
  \vspace{-0.5 cm}
\end{figure*}

% we only visualize the time spans corresponding to the top $K$ confidence scores.
% The green means the ground truth.

==> Figures/overview.tex <==
\begin{figure*}[!ht]
  \centering
  \includegraphics[width=1\linewidth]{Photo/DiffusionVMR_Overview2.pdf}
  \caption{\textbf{Left:} Overview of the proposed DiffusionVMR for joint video moment retrieval and highlight detection tasks. \textbf{Right:} The pipeline of the training and inference of video moment retrieval. The moment retrieval branch comprises a cross-modal encoder and a moment denoising decoder. In the training phase, the GT moment undergoes $t$-step diffusion processes and then is provided to the denoising decoder as the noisy span. Each layer in the denoising decoder takes video representation and noisy span as input, outputting the new span updated by the denoised representation. In inference, the noisy spans are directly sampled from Gaussian noise, and the final output from the decoder is used as the result.}
  \label{fg2}
  \vspace{-0.2 cm}
\end{figure*}

% The cross-modal encoder is used to construct the denoising generation condition, i.e. query-based video representation. The moment denoising decoder comprises $N$ cascading denoising layers that restore the noise proposal span to the target. 

% Overview of the proposed DiffusionVMR for video moment retrieval task. DiffusionVMR comprises a cross-modal encoder and a denoising decoder. The cross-modal encoder is used to construct the denoising generation condition, i.e. query-based video representation. The denoising decoder is composed of $N$ cascading denoising layers that restore the noise proposal span to the target. In the training phase, the target moment undergoes $t$-step random diffusion processes and then is provided to the denoising decoder as the noise proposal span. Each layer in the denoising decoder takes video representation and noise proposal span as input and outputs the new span updated by the denoised representation. In inference, the noise proposal spans are directly sampled from Gaussian noise, and the final output from the decoder is used as the result.

==> Figures/overview_HL.tex <==
%%
%%
\begin{figure}[!t]
  \centering
  \includegraphics[width=1\linewidth]{Photo/DiffusionVMR_HL_Overview.pdf}
  \caption{The pipeline of the highlight detection branch. In each sampling step, the denoising head directly predicts the distribution of $\bm{\hat{x}}_0$ based on $\bm{\hat{x}}_{t}$. For iterative refinement, $\bm{\hat{x}}_{t-1}$ can be derived from $\bm{\hat{x}}_0$ through  Eq.\ref{Diff_infence_diffusion} and serves as the input for the next step.}
  \label{fg_OverviewHL}
  \vspace{-0.1 cm}
\end{figure}

% illustration of the


==> Tables/Charades.tex <==
%
%
\begin{table}[!t]
\centering
\caption{{\upshape Comparisons on the test split of the Charades-STA dataset for video moment retrieval. {Since the proposal spans are randomly initialized from Gaussian noise, the experiment is repeated 5 times at the same checkpoint, with the mean performance and standard reported.} The results presented are obtained at S2@20.}}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{lccc}
\toprule
Method                & Feat.     & R1@0.5         & R1@0.7         \\ \midrule
SAP~\cite{twostage6}        & VGG       & 27.42          & 13.36          \\
SM-RL~\cite{reinforcement2} & VGG & 24.36          & 11.17          \\
TripNet~\cite{tripnet} & VGG       & 36.61          & 14.50          \\
MAN~\cite{anchor2}     & VGG       & 41.24          & 20.54          \\
2D-TAN~\cite{2D-TAN}  & VGG       & 40.94          & 22.85          \\
FVMR~\cite{fvmr}      & VGG       & 42.36          & 24.14          \\
UMT~\cite{UMT}        & VGG+Opti. & 49.35          & 26.16          \\
{CVDN}~\cite{cvdn}      & VGG       & 48.31          & 29.75          \\
{MomentDiff}~\cite{Momentdiff} & VGG       & 51.94          & 28.25   \\
QD-DETR~\cite{qddetr} & VGG       & 52.77          & 31.13          \\
MH-DETR~\cite{mhdetr} & VGG       & \underline{55.47}          & \underline{32.41}          \\
\textbf{DiffusionVMR} & VGG       & $\textbf{57.74}_{\pm 0.11}$ & $\textbf{37.23}_{\pm 0.26}$ \\ \midrule
CAL~\cite{cal}        & SF+C      & 47.31          & 30.19          \\
2D-TAN~\cite{2D-TAN}  & SF+C      & 39.70          & 23.31          \\
VSLNet~\cite{vslnet}  & SF+C      & 47.31          & 30.19          \\
IVG-DCL~\cite{ivgdcl} & SF+C      & 50.24          & 32.88          \\
M-DETR~\cite{moment-detr} & SF+C      & 53.63          & 31.37          \\
{MomentDiff}~\cite{Momentdiff} & SF+C       & 55.57          & 32.42  \\
QD-DETR~\cite{qddetr} & SF+C      & 57.31          & 32.55          \\
UniVTG~\cite{univtg}  & SF+C      & \underline{58.01}          & \underline{35.65}          \\
\textbf{DiffusionVMR} & SF+C      & $\textbf{59.66}_{\pm 0.15}$ & $\textbf{38.73}_{\pm 0.08}$  \\ \bottomrule
\end{tabular}
\vspace{-0.4 cm}
\label{MR_charades}
\end{table}


% Comparisons on the test split of Charades-STA dataset for video moment retrieval. Since the proposal spans are randomly initialized from Gaussian noise, we repeat the experiment 5 times under the same checkpoint and report the mean performance and standard deviation. The best results are in bold and the second-best ones are underlined.

==> Tables/HD_TVSum.tex <==
%% 
\begin{table*}[!t]
\centering
\caption{{\upshape Highlight Detection results of Top-5 mAP on TVSum. $\dagger$ denotes using audio modality. The experiment is repeated 5 times, with the mean performance and standard report. The sampling step is tailored for different domains.}}
\renewcommand{\arraystretch}{1.1}
\renewcommand\tabcolsep{5pt}
\begin{tabular}{lccccccccccc}
\toprule
\multicolumn{1}{c}{\textbf{Method}}     & {VT}    & {VU}   & {GA}   & {MS}   & {PK}   & {PR}   & {FM}   & {BK}   & {BT}   & {DS}   & \textbf{Avg.} \\ \midrule
sLSTM \cite{sLSTM}                        & $41.1$ & $46.2$  & $46.3$ & $47.7$ & $44.8$ & $46.1$ & $45.2$ & $40.6$ & $47.1$ & $45.5$ & $45.1$ \\ 
SG \cite{SG}                              & $42.3$ & $47.2$  & $47.5$ & $48.9$ & $45.6$ & $47.3$ & $46.4$ & $41.7$ & $48.3$ & $46.6$ & $46.2$ \\
LIM-S \cite{lessismore}                   & $55.9$ & $42.9$  & $61.2$ & $54.0$ & $60.4$ & $47.5$ & $43.2$ & $66.3$ & $69.1$ & $62.6$ & $56.3$ \\
Trailer \cite{trailer}                    & $61.3$ & $54.6$  & $65.7$ & $60.8$ & $59.1$ & $70.1$ & $58.2$ & $64.7$ & $65.6$ & $68.1$ & $62.8$ \\
SL-Module \cite{SL_module}                & $86.5$ & $68.7$  & $74.9$ & $\mathbf{86.2}$ & $79.0$ & $63.2$ & ${58.9}$ & ${72.6}$ & ${78.9}$ & $64.0$ & ${73.3}$ \\
UniVTG~\cite{univtg}                    & $83.9$ & $85.1$  & $89.0$ & $80.1$ & $\mathbf{84.6}$ & $81.4$ & $70.9$ & $91.7$ & $73.5$ & $69.3$ & $81.0$ \\ \midrule

MINI-Net$^\dagger$ \cite{miniNet}         & $80.6$ & $68.3$  & $78.2$ & $81.8$ & $78.1$ & $65.8$ & $57.8$ & $75.0$ & $80.2$ & $65.5$ & $73.2$ \\
TCG$^\dagger$ \cite{tcg}                  & $85.0$ & $71.4$  & $81.9$ & $78.6$ & $80.2$ & $75.5$ & $71.6$ & $77.3$ & $78.6$ & $68.1$ & $76.8$ \\
Joint-VA$^\dagger$ \cite{jointVA}         & $83.7$ & $57.3$  & $78.5$ & $86.1$ & $80.1$ & $69.2$ & $70.0$ & $73.0$ & $\mathbf{97.4}$ & $67.5$ & $76.3$ \\
UMT$^\dagger$\cite{UMT}                   & $87.5$ & $81.5$  & $88.2$ & $78.8$ & $81.5$ & $\mathbf{87.0}$ & $\mathbf{76.0}$ & ${86.9}$ & ${84.4}$ & $\mathbf{79.6}$ & ${83.1}$ \\\midrule

\textbf{DiffusionVMR}         & \begin{tabular}[c]{@{}c@{}}{$\mathbf{87.6}$}\\$_{\pm0.01}$\end{tabular} & \begin{tabular}[c]{@{}c@{}}{$\mathbf{93.5}$}\\$_{\pm0.02}$\end{tabular}  & \begin{tabular}[c]{@{}c@{}}{$\mathbf{94.1}$}\\$_{\pm0.02}$\end{tabular}  & \begin{tabular}[c]{@{}c@{}}{84.9}\\$_{\pm0.01}$\end{tabular}  & \begin{tabular}[c]{@{}c@{}}{79.4}\\$_{\pm0.05}$\end{tabular}  & \begin{tabular}[c]{@{}c@{}}{79.6}\\$_{\pm0.02}$\end{tabular}  & \begin{tabular}[c]{@{}c@{}}{66.8}\\$_{\pm0.04}$\end{tabular}  & \begin{tabular}[c]{@{}c@{}}{$\mathbf{92.9}$}\\$_{\pm0.02}$\end{tabular}  & \begin{tabular}[c]{@{}c@{}}{85.8}\\$_{\pm0.01}$\end{tabular}  & \begin{tabular}[c]{@{}c@{}}{$\mathbf{79.6}$}\\$_{\pm0.03}$\end{tabular}  & $\mathbf{84.4}$ \\   \bottomrule

\end{tabular}
\vspace{-0.1 cm}
\label{HL_TVSum}
\end{table*}

==> Tables/HD_YouTubeHL.tex <==
%% 
\begin{table}[!t]
\centering
\caption{{\upshape Highlight Detection results of mAP on YouTube HL. $\dagger$ denotes using audio modality. The sampling step is tailored for different domains.}}
\renewcommand{\arraystretch}{1.1}
\renewcommand\tabcolsep{4.05pt}
\begin{tabular}{lccccccc}
\toprule
\multicolumn{1}{c}{\textbf{Method}}    & Dog     & Gym.        & Par.     & Ska.    & Ski.     & Sur.     & \textbf{Avg.} \\ \midrule
RRAE \cite{RRAE}              & 49.0    & 35.0        & 50.0     & 25.0    & 22.0     & 49.0     & 38.3 \\  
GIFs \cite{Video2gif}         & 30.8    & 33.5        & 54.0     & 55.4    & 32.8     & 54.1     & 46.4\\
LSVM~\cite{youtube}           & 60.0    & 41.0        & 61.0     & 62.0    & 36.0     & 61.0     & 53.6\\
LIM-S~\cite{lessismore}       & 57.9    & 41.7        & 67.0     & 57.8    & 48.6     & 65.1     & 56.4 \\
SL-Module~\cite{SL_module}    & 70.8    & 53.2        &77.2      & 72.5    & 66.1     & 76.2     & 69.3 \\
QD-DETR~\cite{qddetr}         & 72.2    & 77.4        & 71.0   & 72.7    & 72.8     & 80.6     & 74.4 \\
UniVTG~\cite{univtg}          & 71.8    & 76.5        & 73.9     &73.3     & 73.2     & 82.2     & 75.2 \\ \midrule
MINI-Net$^\dagger$~\cite{miniNet}    & 58.2    & 61.7        & 70.2     &72.2     & 58.7     & 65.1     & 64.4 \\
TCG$^\dagger$~\cite{tcg}      & 55.4    & 62.7        & 70.9     & 69.1    & 60.1     & 59.8     & 63.0 \\
Joint-VA$^\dagger$~\cite{jointVA}    & 64.5    & 71.9        & 80.8     & 62.0    & 73.2     & 78.3     & 71.8 \\
UMT$^\dagger$~\cite{UMT}      & 65.9    & 75.2    &\textbf{81.6}  & 71.8   & 72.3 &\textbf{82.7} & 74.9 \\ \midrule
\textbf{DiffusionVMR}         & \begin{tabular}[c]{@{}c@{}}{\textbf{74.1}}\\$_{\pm0.01}$\end{tabular} & \begin{tabular}[c]{@{}c@{}}{\textbf{78.7}}\\$_{\pm0.01}$\end{tabular}  & \begin{tabular}[c]{@{}c@{}}{74.2}\\$_{\pm0.03}$\end{tabular}  & \begin{tabular}[c]{@{}c@{}}{\textbf{73.8}}\\$_{\pm0.01}$\end{tabular}  & \begin{tabular}[c]{@{}c@{}}{\textbf{73.9}}\\$_{\pm0.02}$\end{tabular}  & \begin{tabular}[c]{@{}c@{}}{80.8}\\$_{\pm0.02}$\end{tabular}  & \textbf{75.9}  \\   \bottomrule
\end{tabular}
\vspace{-0.3 cm}
\label{HL_YouTube}
\end{table}

==> Tables/TACoS.tex <==
\begin{table}[t]
\centering
\caption{{\upshape Comparisons on the test split of the TACoS dataset for video moment retrieval. {The experiment is repeated 5 times, with the mean performance and standard report.} The results presented are obtained at S2@20.}}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{lcccc}
\toprule
Method                       & Feat.          & R1@0.1 & R1@0.3 & R1@0.5 \\ \midrule
MCN~\cite{twostage2}         & C3D          & 14.42  & -      & 5.58   \\
CTRL~\cite{twostage1}        & C3D          & 24.32  & 18.32  & 13.30  \\
TGN~\cite{anchor1}           & C3D          & 41.87  & 21.77  & 18.90  \\
%ACRN~\cite{acrn}             & C3D          & 24.22  & 19.52  & 14.62  \\
ACL-K~\cite{aclk}            & C3D          & 31.64  & 24.17  & 20.01  \\
CMIN~\cite{cmin}             & C3D          & 36.68  & 27.33  & 19.57  \\
SM-RL~\cite{reinforcement2}  & C3D          & 26.51  & 20.25  & 15.95  \\
SLTA~\cite{slta}             & C3D          & 23.13  & 17.07  & 11.92  \\
SAP~\cite{twostage6}               & C3D          & 31.15  & -      & 18.24  \\
TripNet~\cite{tripnet}       & C3D          & -      & 23.95  & 19.17  \\
2D-TAN~\cite{2D-TAN}         & C3D          & 47.59  & 37.29  & 25.32  \\
CSMGAN~\cite{csmgan}         & C3D          & 42.74  & 33.90  & 27.09  \\
FIAN~\cite{fian}             & C3D          & 39.55  & 33.87  & 28.58  \\
LGN~\cite{lgn}               & C3D          & 52.46  & 41.71  & 30.57  \\
SMRN~\cite{smrn}             & C3D          & 50.44  & 42.49  & 32.07  \\
{MomentDiff}~\cite{Momentdiff} & C3D          & 56.81  & 44.78  & 33.68  \\
VLG-Net~\cite{vlgnet}        & C3D          & \underline{57.21}  & \underline{45.46}  & \underline{34.19}  \\
\textbf{DiffusionVMR}        & C3D          & $\textbf{58.57}_{\pm 0.17}$  & $\textbf{47.41}_{\pm 0.14}$  & $\textbf{36.79}_{\pm 0.27}$  \\ \midrule
2D-TAN~\cite{2D-TAN}         & SF+C         & -      & 40.01  & 27.99  \\
VSLNet~\cite{vslnet}         & SF+C         & -      & 35.54  & 23.54  \\
M-DETR~\cite{moment-detr}    & SF+C         & -      & 37.97  & 24.67  \\
UniVTG~\cite{univtg}         & SF+C         & -      & \underline{51.44}  & \underline{34.97}  \\
\textbf{DiffusionVMR} & SF+C         & $\textbf{63.84}_{\pm 0.12}$  & $\textbf{52.90}_{\pm 0.06}$  & $\textbf{38.02}_{\pm 0.19}$  \\ \bottomrule
\end{tabular}
\vspace{-0.4 cm}
\label{MR_tacos}
\end{table}



==> Tables/oneLine_HD.tex <==
%% 
\begin{figure*}[t]
\begin{minipage}[t]{0.6\textwidth}
\centering
\scriptsize
\caption{{\upshape Highlight Detection results of mAP on YouTube HL. $\dagger$ denotes using audio modality.}}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{lccccccc}
\toprule
\multicolumn{1}{c}{\textbf{Method}}    & Dog     & Gym.        & Par.     & Ska.    & Ski.     & Sur.     & \textbf{Avg.} \\ \midrule
RRAE \cite{}                  & 49.0    & 35.0        & 50.0     & 25.0    & 22.0     & 49.0     & 38.3 \\  
GIFs \cite{}                  & 30.8    & 33.5        & 54.0     & 55.4    & 32.8     & 54.1     & 46.4\\
LSVM~\cite{}                  & 60.0    & 41.0        & 61.0     & 62.0    & 36.0     & 61.0     & 53.6\\
LIM-S~\cite{}                 & 57.9    & 41.7        & 67.0     & 57.8    & 48.6     & 65.1     & 56.4 \\
SL-Module~\cite{}             & 70.8    & 53.2        &77.2      & 72.5    & 66.1     & 76.2     & 69.3 \\
QD-DETR~\cite{}               & 72.2    & \textbf{77.4} & 71.0   & 72.7    & 72.8     & 80.6     & 74.4 \\
UniVTG~\cite{}                & 71.8    & 76.5        & 73.9     &73.3     & 73.2     & 82.2     & 75.2 \\ \midrule
MINI-Net$^\dagger$~\cite{}    & 58.2    & 61.7        & 70.2     &72.2     & 58.7     & 65.1     & 64.4 \\
TCG$^\dagger$~\cite{}         & 55.4    & 62.7        & 70.9     & 69.1    & 60.1     & 59.8     & 63.0 \\
Joint-VA$^\dagger$~\cite{}   & 64.5    & 71.9        & 80.8     & 62.0    & 73.2     & 78.3     & 71.8 \\
UMT$^\dagger$~\cite{}         & 65.9    & 75.2    &\textbf{81.6}  & 71.8   & 72.3 &\textbf{82.7} & 74.9 \\ \midrule
\textbf{DiffusionVMR}         & \begin{tabular}[c]{@{}c@{}}{00.0}\\$_{\pm0.00}$\end{tabular} & \begin{tabular}[c]{@{}c@{}}{00.0}\\$_{\pm0.00}$\end{tabular}  & \begin{tabular}[c]{@{}c@{}}{00.0}\\$_{\pm0.00}$\end{tabular}  & \begin{tabular}[c]{@{}c@{}}{00.0}\\$_{\pm0.00}$\end{tabular}  & \begin{tabular}[c]{@{}c@{}}{00.0}\\$_{\pm0.00}$\end{tabular}  & \begin{tabular}[c]{@{}c@{}}{00.0}\\$_{\pm0.00}$\end{tabular}  & \begin{tabular}[c]{@{}c@{}}{00.0}\\$_{\pm0.00}$\end{tabular}  \\   \bottomrule

\end{tabular}
\end{minipage}

\begin{minipage}[t]{0.3\textwidth}
\centering
\begin{figure}
  % \centering
  \includegraphics[width=0.3\linewidth]{Photo/increase_proposals_5.pdf}
  \caption{Effectiveness of different numbers of proposals on QVHighlights val split. The training and inference of DiffusionVMR are decoupled. As the number of proposals in inference increases, the performance of DiffusionVMR improves steadily.}
  \label{fg3}
\end{figure}

\end{minipage}
\end{figure*}
